Hard isogeny problems over RSA moduli and groups with infeasible inversion

We initiate the study of computational problems on elliptic curve isogeny graphs defined over RSA moduli. We conjecture that several variants of the neighbor-search problem over these graphs are hard, and provide a comprehensive list of cryptanalytic attempts on these problems. Moreover, based on the hardness of these problems, we provide a construction of groups with infeasible inversion, where the underlying groups are the ideal class groups of imaginary quadratic orders. Recall that in a group with infeasible inversion, computing the inverse of a group element is required to be hard, while performing the group operation is easy. Motivated by the potential cryptographic application of building a directed transitive signature scheme, the search for a group with infeasible inversion was initiated in the theses of Hohenberger and Molnar (2003). Later it was also shown to provide a broadcast encryption scheme by Irrer et al. (2004). However, to date the only case of a group with infeasible inversion is implied by the much stronger primitive of self-bilinear map constructed by Yamakawa et al. (2014) based on the hardness of factoring and indistinguishability obfuscation (iO). Our construction gives a candidate without using iO.

==> fig_volcano_example.tex <==

\begin{figure}
  \centering
    \begin{tikzpicture}
      \begin{scope}[xshift= 9.7 cm]
      \node at (0, -1.5) {$\overrightarrow{CRT}$};
      \end{scope}
      \begin{scope}[xshift= 13 cm]
        \def\crater{7}
        \foreach \i in {1,...,\crater} {
          \draw[fill] (360/\crater*\i:1cm) circle (1pt);
          \draw (360/\crater*\i : 1cm) -- (360/\crater*\i+360/\crater : 1cm);
                    \node at (0,0) {$\Z_{14359}$};
                    \node at (-1.9, 0.7) {$j_0 = 12631$};
                    \node at (-0.3, 1.6) {$j_1 = 7601$};
                    \node at ( 1.2, 1.3) {$j_2 = 1766$};
                    \node at ( 2.05, 0.0) {$j_3 = 4096$};
                    \node at ( 1.2,-1.3) {$j_4 = 7919$};
                    \node at (-0.4,-1.6) {$j_5 = 2711$};
                    \node at (-1.9,-0.7) {$j_6 = 1897$};
        }
      \end{scope}
    \end{tikzpicture}
    \caption{A representation of $\CL(-251)$ by a $3$-isogeny volcano over $\Z_{14359}$ of size $h(-251)=7$. The volcano is composed by fixing $j_0 = \CRT(15, 2; 83, 173) = 12631$, and let $(j_0, 7601)$ represent the ideal class $[(3, a, \cdot)]$ for some $a\in\Z$, which fixes the rest of the action (e.g. $(j_0, 1897)$ represents $[(3, -a, \cdot)]$). 
    %From the integers over $\F_{83}$ and $F_{173}$. Let $j_0 = \CRT(15, 2)$. [15, 48, 23, 29, 34, 55, 71]; over $\F_{173}$: [2, 162, 36, 117, 134, 116, 167]. Over $N = 14359$: [12631, 7601, 1766, 4096, 7919, 2711, 1897]. 
    }\label{fig:volcano_example}
\end{figure}

==> sec_30_cryptanalysis.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  
%  Cryptanalysis
%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Cryptanalysis}\label{sec:cryptanalysis}

We provide a highlight of the cryptanalytic attempts we have made and discuss the impacts and the countermeasures. The details of our cryptanalysis attempts can be found in the full version in the supplementary material. 

The security of our cryptosystem relies on the conjectured hardness of solving various problems over $\ZNZ$ without knowing the factors of $N$. So we start from the feasibility of performing several individual computational tasks over $\ZNZ$; then focus on the $(\ell, \ell^2)$-isogenous neighbor problem over $\ZNZ$, whose hardness is necessary for the security of our candidate TGII; finally address all the other attacks in the TGII construction.

\subsection{The (in)feasibility of performing computations over $\ZNZ$}

{\bf Factoring polynomials over $\ZNZ$.} 
The task of finding roots of polynomials of degree $d \geq2$ over $\ZNZ$ sits in the subroutines of many potential algorithms we need to consider, so let us begin with a clarification on the status of this problem. No polynomial time algorithm is known to solve this problem in general. In a few special cases, finding at least one root is feasible. For example, if a root of a polynomial over $\ZNZ$ is known to be the same as the root over $\Q$, then we can use LLL \cite{lenstra1982factoring}; or if a root is known to be smaller than roughly $O(N^{1/d})$, then Coppersmith-type algorithms can be used to find such a root \cite{DBLP:journals/joc/Coppersmith97}. However, these families of polynomials only form a negligible portion of all the polynomials with polynomially bounded degrees. 

\subsubsection{Feasible information from a single $j$-invariant}
From any $j \in \ZNZ, j\neq 0,1728$, we can find the coefficients $a$ and $b$ of the Weierstrass form of an elliptic curve $E(\ZNZ)$ with $j(E) = j$ by computing $a=3j(1728-j), b = 2j(1728-j)^2$. %However, this method does not guarantee that the curve belongs to a specific isomorphism class (there are four of them). By choosing a value $u \in (\ZNZ)^{\times}$ and let $a^* = u^4  a, b^* = u^6  b$ one gets the coefficient of another curve with the same $j$-invariant, each belonging to one of the four isomorphism classes.
But choosing a curve over $\ZNZ$ with a given $j$-invariant together with a point on the curve seems tricky. Nevertheless, it is always feasible to choose a curve together with the $x$-coordinate of a point on it, since a random $x \in \ZNZ$ is the $x$-coordinate of some point on the curve with probability roughly
$\frac12$. It is also known that computing the multiples of a point $P$ over $E(\ZNZ)$ is feasible solely using the $x$-coordinate of $P$ (cf. \cite{DBLP:conf/eurocrypt/Demytko93}). The implication of this is that we should at the very least not give out the group orders of the curves involved in the scheme. More precisely, we should avoid the $j$-invariants corresponding to curves (or their twists) with polynomially smooth cardinalities over either $\F_p$ or $\F_q$. Otherwise Lenstra's algorithm \cite{lenstra1987factoring} can be used to factorize $N$. 

In our application we also assume that the endomorphism rings of $E(\F_p)$ and $E(\F_q)$ are isomorphic and not given out (the reason will be explained later). Computing the discriminant of $\OOO \simeq \Endo(E(\F_p)) \simeq \Endo(E(\F_q))$ or the number of points of $E$ over $\Z/N\Z$ seems to be hard given only $N$ and a $j$-invariant. In fact Kunihiro and Koyama (and others) have reduced factorizing $N$ to computing the number of points of general elliptic curves over $\Z/N\Z$ \cite{DBLP:conf/eurocrypt/KunihiroK98}. However, these reductions are not efficient in the special case, where the endomorphism rings of $E(\F_p)$ and $E(\F_q)$ are required to be isomorphic. 
So, the result of \cite{DBLP:conf/eurocrypt/KunihiroK98} can be viewed as evidence that the polynomial time algorithms for counting points on elliptic curves over finite fields may fail over $\Z/N\Z$ without making use of the fact that the endomorphism rings of $E(\F_p)$ and $E(\F_q)$ are isomorphic.

Let $\ell$ be a prime. We will be concerned with degree $\ell$ isogenies. If we are only given a single $j$-invariant $j_1 \in\Z/N\Z$, then finding an integer $j_2$ such that $\Phi_\ell(j_1, j_2) = 0 \pmod N$ seems hard. Nevertheless, we remark that Theorem~\ref{thm:basicequalfactoring} does not guarantee that finding $j_2$ is as hard as factoring when the endomorphism rings of $E(\F_p)$ and $E(\F_q)$ are isomorphic. However, as of now, we do not know how to make use of the condition that the endomorphism rings are isomorphic to mount an attack on the problem.

\subsubsection{Feasible information from more $j$-invariants} 
In the construction of a TGII we are not only given a single $j$-invariant, but many $j$-invariants with each neighboring pair of them satisfying the $\ell^{th}$ modular polynomial, a polynomial degree $\ell + 1$. We will study what other information can be extracted from these neighboring $j$-invariants.

In Proposition~\ref{claim:kernelpoly}, we have explained that given two integers $j_1, j_2\in\ZNZ$ such that $\Phi_{\ell}(j_1, j_2) = 0$ over $\ZNZ$, the elliptic curves $E_1$, $E_2$, and the kernel polynomial $h(x)$ of an isogeny $\phi$ from $E_1$, $E_2$ can be computed in time polynomial in $\ell, \log(N)$. However, it is not clear how to use the explicit expression of $\phi$ to break factoring or solve the inversion problem. 

A natural next step is to recover a point in the kernel of $\phi$, but it is also not clear how to recover even the $x$-coordinate of a point in the kernel when $\ell \geq 5$. For $\ell=3$, on the other hand, the kernel polynomial does reveal the $x$-coordinate of a point $P$ in the kernel $G\subset E_1[3]$ (note that $h(\cdot)$ is of degree $1$ in this particular case). But revealing the $x$-coordinate of a point $P\in E_1[3]$ does not immediately break factoring, since $3P$ is $O$ over both $\F_p$ and $\F_q$. At this moment we do not know of a full attack from a point in $\ker(\phi)$. Nevertheless, we still choose to take an additional safeguard by avoiding the use of 3-isogenies since it reveals the $x$-coordinate of a point in $E_1[3]$, and many operations on elliptic curves are feasible given the $x$-coordinate of a point.

\subsection{Tackling the $(\ell, \ell^2)$-isogenous neighbor problem over $\ZNZ$}\label{sec:analysis_ell_ell2}

The $(\ell, \ell^2)$-isogenous neighbor problem is essential to the hardness of inversion in our TGII construction. In addition to Definition~\ref{def:problem:joint}, we assume that the endomorphism rings of the curves in the problem are isomorphic to an imaginary quadratic order $\OOO$. 

\subsubsection{The Hilbert class polynomial attack}
We first note that the discriminant $D$ of the underlying endomorphism ring $\OOO$ cannot be polynomially large, otherwise we can compute the Hilbert class polynomial $H_D$ in polynomial time and therefore solve the $(\ell, \ell^2)$-isogenous neighbor problem. 
Given $j_0, j_1$ such that $\Phi_\ell(j_0, j_1) = 0$, compute the polynomial $\gamma(x)$,
\[ \gamma(x) := \gcd( \Phi_{\ell}(j_0, x), \Phi_{\ell^2}(j_1, x), H_{D}(x) ) \in(\ZNZ)[x] .\] 
The gcd of $\Phi_{\ell}(j_0, x)$ and $\Phi_{\ell^2}(j_1, x)$ gives a polynomial of degree $\ell$. The potential root they share with $H_{D}(x)$ is the only one with the same endomorphism ring with $j_0$ and $j_1$, which is $j_{-1}$. So $\gamma(x)$ is a linear function. 

\subsubsection{Survey of the Ionica-Joux algorithm }
Among the potential solutions to the $(\ell, \ell^2)$-isogenous neighbor problem, finding the one corresponding to the image of a horizontal isogeny would break our candidate group with infeasible inversion, so it is worth investigating algorithms which find isogenies with specific directions. However, the only known such algorithm over the finite fields, that of Ionica and Joux \cite{DBLP:journals/moc/IonicaJ13}, does not seem to work over $\ZNZ$. In the full version we provide a detailed survey of this algorithm.

\subsubsection{More about modular curves and characteristic zero attacks}
Given $j$, solving $\Phi_{\ell}(j,x)$ is not the only way to find the $j$-invariants of the $\ell$-isogenous curves. Alternative complex analytic (i.e. characteristic zero) methods have been discussed, for instance, in \cite[Section~3]{elkies1998elliptic}. However, these methods all involve solving polynomials of degree $\geq2$ to get started.

As mentioned in Section~\ref{sec:prelim:isogeny}, the curve $\uhp/\Gamma_0(\ell)$ parameterizes pairs of elliptic curves over $\C$ related by a cyclic $\ell$-isogeny. The $(\ell,\ell^2)$-isogenous neighbor problem, on the other hand, concerns curves that are horizontally $\ell$-isogenous, i.e. $\ell$-isogenous and have the same endomorphism ring. To avoid an attack through characteristic zero techniques, we make sure that there is no immediate quotient of $\uhp$ that parametrizes curves which are related with an $\ell$-isogeny and have the same endomorphism ring. Below, we first go over the well-known moduli description of modular curves to make sure that they don't lead to an immediate attack, and then show that there is indeed no quotient of $\uhp$ between $\uhp/\SL_2(\Z)$ and $\uhp/\Gamma_0(\ell)$, so we don't have to worry about possible attacks on that end. 

Let $\Gamma: = \SL_2(\Z)$, and let $\Gamma(\ell)$ and $\Gamma_1(\ell)$ denote the congruence subgroups,

 %The quotient $\uhp/\Gamma$ is known as the modular curve $Y(1)$, and $X(1) = \uhp^*/\Gamma$. %$\Gamma(1) = \SL_2(\Z)/\set{\pm 1} $
\[ \Gamma(\ell):=\set{ \pmat{ a & b \\ c & d  }\in\SL_2(\Z) \bigg\vert \pmat{ a & b \\ c & d  } \equiv \pmat{ 1 & 0 \\ 0 & 1  }\pmod \ell  }, \]
\[ \Gamma_1(\ell):=\set{ \pmat{ a & b \\ c & d  }\in\SL_2(\Z) \bigg\vert \pmat{ a & b \\ c & d  } \equiv \pmat{ 1 & * \\ 0 & 1  }\pmod \ell  }. \]
%\[ \Gamma_0(\ell):=\set{ \pmat{ a & b \\ c & d  }\in\SL_2(\Z) \bigg\vert \pmat{ a & b \\ c & d  } \equiv \pmat{ * & * \\ 0 & *  }\pmod \ell  }. \]

It is well-known that the curves $\uhp/\Gamma_1(\ell)$ and $\uhp/\Gamma(\ell)$ parametrize elliptic curves with extra data on their $\ell$-torsion (cf. \cite{kohel1996endomorphism}). $\uhp/\Gamma_1(\ell)$ parametrizes $(E, P)$, where $P$ is a point on $E$ having order exactly $\ell$, and $\uhp/\Gamma(\ell)$ parametrizes triples $(E,P,Q)$, where $E[\ell]=\langle P,Q\rangle$ and they have a fixed Weil pairing. These curves carry more information than the $\ell$-isogenous relation and they are not immediately helpful for solving the $(\ell, \ell^2)$-isogenous neighbor problem.
%If we need a reference for this \cite{Diamond:2005aa} \S7 is a good one.

As for the quotients between $\uhp/\SL_2(\Z)$ and $\uhp/\Gamma_0(\ell)$, the following lemma shows that there are indeed none.
%From \cite[Page~86]{silverman2013advanced} we have $[ \Gamma : \Gamma_0(\ell) ] = \ell \prod_{p\mid \ell}\left( 1+1/p \right) $, which does not rule out the chance of having a subgroup between $\Gamma$ and $\Gamma_0(\ell)$.

%\ynote{TBD: explore the possible subgroups between $\Gamma$ and $\Gamma_0(\ell)$, see if they matters}

%\anote{I believe there is no such subgroup so we are good. Here is an argument:}

\begin{lemma}
Let $\ell$ be a prime. If $H\leq \Gamma$ is such that $\Gamma_0(\ell)\leq H\leq \Gamma$, then either $H=\Gamma_0(\ell)$ or $H=\Gamma$.
\end{lemma}
\begin{proof} Let $\sigma_1=\left(\begin{smallmatrix}1&1\\0&1\end{smallmatrix}\right)$, $\sigma_2=\left(\begin{smallmatrix}1&0\\1&1\end{smallmatrix}\right)$, $\sigma_3=\sigma_1\sigma_2^{-1}$, and recall that $SL_2(\Z/\ell\Z)=\langle\sigma_1,\sigma_2\rangle=\langle\sigma_1,\sigma_3\rangle$. Recall that the natural projection $\pi: \Gamma \rightarrow SL_2(\Z/\ell\Z)$ is surjective. Assume that $H\neq \Gamma_0(\ell)$. This implies that $\pi(H)=SL_2(\Z/\ell\Z)$ (we shall give a proof below). Assuming this claim for the moment let $g\in \Gamma\backslash H$. Since $\pi(\Gamma)=\pi(H) $ there exists $h\in H$ such that $\pi(g)=\pi(h)$. Therefore, $gh^{-1}\in \ker(\pi)=\Gamma(\ell)\subset H$. Therefore, $g\in H$ and $\Gamma=H$.

To see that $\pi(\Gamma)=\pi(H)$, first note that since $\Gamma_0(\ell) \subset H$ we have  all the upper triangular matrices in $ \pi(H)$. Next, let $h=\left(\begin{smallmatrix}h_1&h_2\\h_3&h_4\end{smallmatrix}\right)\in H\backslash \Gamma_0(\ell)$ such that $\pi(h)=\left(\begin{smallmatrix}\bar{h}_1&\bar{h}_2\\ \bar{h}_3&\bar{h}_4\end{smallmatrix}\right)\in \pi(H)\backslash \pi(\Gamma_0(\ell))$ (note that this difference is non-empty since otherwise $\Gamma_0(\ell)=H$). \\
We have two cases depending on $\bar{h}_1= 0$ or not. If $\bar{h}_1=0$ then $\bar{h}_3\neq0$ and $\sigma_3=\left(\begin{smallmatrix}\bar{h}_3^{-1}&\bar{h}_4\\ 0&\bar{h}_3\end{smallmatrix}\right)\bar{h}^{-1}\in \pi(H)$. On the other hand, if $\bar{h}_1\neq0$ multiplying on the right by $\left(\begin{smallmatrix}\bar{h}_1^{-1}&-\bar{h}_2\\0&\bar{h}_1\end{smallmatrix}\right) \in \pi(H)$ we see that $\left(\begin{smallmatrix}1&0\\ \bar{h}_3\bar{h}_1^{-1}&1\end{smallmatrix}\right) \in \pi(H)$ . For any integer $m$, the $m$'th power of this matrix is $\left(\begin{smallmatrix}1&0\\ m\bar{h}_3\bar{h}_1^{-1}&1\end{smallmatrix}\right) \in \pi(H)$. Taking $m\equiv \bar{h}_1\bar{h}_3^{-1}$ shows that $\sigma_2\in \pi(H)$. This shows that $\pi(H)=SL_2(\Z/\ell\Z)$.
\end{proof}

%Let us also remark that for special values of $\ell$ the $(\ell,\ell^2)$-isogenous neighbor problem may be more prone to characteristic zero attacks (although we do not know of such an attack). For instance, for those $\ell$ for which $\uhp/\Gamma_0(\ell)$ (more precisely, its compactification $X_0(\ell)$) is genus $0$ or $1$, it (may) have many rational points. These points, in turn, can be used to get points over $\ZNZ$ without knowing the factorization of $N$. Nevertheless, we may just avoid these values in the system. As mentioned above, we currently do not see an attack based on this. This point is brought up just as an extra precautionary measure.
\iffalse
We have also been looking into the potential characteristic zero attacks using the modular curves. So far we haven't found any modular congruence subgroups that characterize horizontal isogenies. When $\ell$ is small the rational points on $X_0(\ell)$ or $X_0(\ell^2)$ might give a way of solving the $(\ell, \ell^2)$-isogenous neighbor problem over $\ZNZ$. We haven't seen a concrete attack using the rational points on the modular curves, but as a precautionary measure, we can choose to use larger $\ell$ (say $\ell>7$) to prevent the potential attacks.
\fi


\subsection{Cryptanalysis of the candidate group with infeasible inversion}\label{sec:attack_concrete_TGII}

We now cryptanalyze the concrete candidate TGII. Recall the format of an encoding of a group element $x$ from Definition~\ref{def:represent_enc}:
\[ \enc(x) = (L_x; T_{x,1}, ..., T_{x,w_x}) = ((p_{x,1}, ..., p_{x,w_x}); (j_{x,1,1}, ..., j_{x,1,e_{x,1}}), ..., (j_{x,w_x,1}, ..., j_{x,w_x,e_{x,w_x}}) ) .\]
The ``exponent vector" $\ary{e}_x\in\Z^{w_x}$ can be read from the encoding as $ \ary{e}_x = ( |T_{x,1}|, ..., |T_{x,w_x}| )$. 

We assume polynomially many composable encodings are published in the applications of a TGII. In down-to-earth terms it means the adversary is presented with polynomially many $j$-invariants on the crater of a volcano, and the explicit isogenies between each pair of the neighboring $j$-invariants (due to Proposition~\ref{claim:kernelpoly}). 

%\paragraph{The ``GCD" attack model.}
We will be considering the following model on the adversary's attacking strategy. 
\begin{definition}[The GCD attack model]\label{def:gcd_eval}
In the GCD attack model, the adversary is allowed to try to find the inverse of a target group element only by executing the unit gcd operation $\gcdop(\PP, \ell_1, \ell_2; j_1, j_2)$ given in Algorithm~\ref{alg:gcdop} for polynomially many steps, where $\ell_1, \ell_2; j_1, j_2$ are from the published encodings or obtained from the previous executions of the gcd evaluations.
\end{definition}
We do not know how to prove the construction of TGII is secure even if the adversary is restricted to attack in the GCD model. Our cryptanalysis attempts can be classified as showing (1) how to prevent the attacks that obey the GCD evaluation law\ifnum\eprint=1  ~(mainly in \S\ref{sec:attack_concrete_TGII_trivial} and \S\ref{sec:parallelogram_attack}); \else; \fi (2) how to prevent the other attack approaches (by e.g. guessing the class group invariants). 

\subsubsection{Preventing the trivial leakage of inverses}\label{sec:attack_concrete_TGII_trivial}
In applications we are often required to publish the encodings of elements that are related in some way. A typical case is the following: for $x, y\in\CL(\OOO)$, the scheme may require publishing the encodings of $x$ and $z = y\circ x^{-1}$ without revealing a valid encoding of $x^{-1}$. As a toy example, let $x = [(p_x, b_x, \cdot)]$, $y = [(p_y, b_y, \cdot)]$, where $p_x$ and $p_y$ are distinct primes. Let $j_0$, the $j$-invariant of a curve $E_0$, represent the identity element in the public parameter. Let $((p_x); (j_x))$ be a composable encoding of $x$ and $((p_y); (j_y))$ be a composable encoding of $y$.

Naively, a composable encoding of $z = y\circ x^{-1}$ could then be $((p_x, p_y); (j_{x^{-1}}), (j_{y}))$, where $j_{x^{-1}}$ is the $j$-invariant of $E_{x^{-1}} = x^{-1}E_0$. Note, however, that $((p_x); (j_{x^{-1}}))$ is a valid encoding of $x^{-1}$. In other words such an encoding of $y\circ x^{-1}$ trivially reveals the encoding of $x^{-1}$. 

One way of generating an encoding of $z = y\circ x^{-1}$ without trivially revealing $j_{x^{-1}}$ is to first pick a generator set of ideals where the norms of the ideals are coprime to $p_x$ and $p_y$, then solve the discrete-log of $z$ over these generators to compute the composable encoding. This is the approach we take in this paper.

%What about $\frac{a+b}{2}$ attack? $\frac{a+b}{2}$ shall be okay, since even computing $a+b$ is okay.

%what about $\frac{a-b}{2}$? This should have been prevented by the same mechanism that prevents $a+b$.

\subsubsection{Parallelogram attack}\label{sec:parallelogram_attack}
In the applications we are often required to publish the composable encodings of group elements $a$, $b$, $c$ such that $a\circ b = c$. If the degrees of the three encodings are coprime, then we can recover the encodings of $a^{-1}$, $b^{-1}$, and $c^{-1}$ using the following ``parallelogram attack". This is a non-trivial attack which obeys the gcd evaluation law in Definition~\ref{def:gcd_eval}.

Let us illustrate the attack via the examples in Figure~\ref{fig:parallelogram}, where the solid arrows represent the isogenies that are given as the inputs (the $j$-invariants of the target curves are written at the head of the arrows, their positions do not follow the relative positions on the volcano; the degree of the isogeny is written on the arrow); the dashed lines and the $j$-invariants on those lines are obtained from the gcd evaluation law. 

\input{fig_parallelogram.tex}

For simplicity let us first look at the example in the left figure. Let composable encodings of $a$, $b$, $c$ be given by $(\ell_1; (j_1))$, $(\ell_2; (j_2))$, $(\ell_3; (j_3))$, where $\ell_1$, $\ell_2$, $\ell_3$ are polynomial and pairwise coprime. 
A composable encoding of $b^{-1}$ then can be written as $(\ell_2; (j_4))$, where $j_4$ is the root of the linear equation $f(x) = \gcd( \Phi_{\ell_3}(j_1, x) , \Phi_{\ell_2}(j_0, x) )$. This is due to the relation $c\circ b^{-1} = a$, which, in particular implies that $j_1$ and $j_4$ are connected by an isogeny of degree $\ell_3$. 

The simple attack above uses the fact that the degrees of the entire encodings of $a$, $b$ and $c$ are polynomial. Let us use the example in the right figure to illustrate that even if the encodings are composed of many polynomial degree isogenies (so that the total degrees may be super-polynomial), the attack is still effective.
The idea is to view the composition law as filling the missing edges of a parallelogram given the $j$-invariants on a pair of adjacent edges. 
The final goal is to find the missing corner $j_{12}$ in the parallelogram $j_0 - j_3 - j_1 - j_{12}$. To arrive there we need the $j$-invariants on a pair of adjacent edges to begin with, so we first have to fill the $j$-invariants on, for instance, the edge $j_1-j_3$. 
Therefore, as the first step, we consider the parallelogram $j_0 - j_2 - j_3 - j_1$. To fill the $j$-invariants on the edge $j_1 - j_3$, we first compute $j_7$ as the root of $f_7(x) = \gcd( \Phi_{\ell_4}(j_5, x) , \Phi_{\ell_5}(j_4, x) )$, then compute $j_8$ as the root of $f_8(x) = \gcd( \Phi_{\ell_1}(j_7, x) , \Phi_{\ell_5}(j_1, x) )$ (the polynomials $f_7$, $f_8$ are linear since the degrees of $\enc(a)$ and $\enc(b)$ are coprime).
In the second step, we consider the parallelogram $j_0 - j_3 - j_1 - j_{12}$. To find $j_{12}$ we use the gcd evaluation law to find $j_9$, $j_{10}$, $j_{11}$, $j_{12}$ one-by-one (using the condition that the degrees of $\enc(c)$ and $\enc(b)$ are coprime). 

The parallelogram attack is very powerful, in the sense that it is not preventable when application requires to publish the composable encodings of $a$, $b$, $c$ such that $a\circ b = c$, and $\enc(a)$, $\enc(b)$, $\enc(c)$ to be pairwise composable. However, the parallelogram attack does not seem to work when 2 out of the 3 pairs of $\enc(a)$, $\enc(b)$ and $\enc(c)$ are not composable. In the applications of directed transitive signature and broadcast encryption, there are encodings of $a$, $b$, $c$ such that $a\circ b = c$. Luckily, only one pair of the encodings among the three has to be composable to provide the necessary functionalities of these applications. %We will explicitly mention how to choose the prime factors in the degrees of these encodings to prevent the parallelogram attack.
%We can recover all the explicit isogenies between neighboring $j$-invariants. Given that we choose all the prime degrees $\ell$ of the isogenies to be $\geq 5$ (or $>7$ for extra precaution), the explicit isogenies do not trivially leak the $x$-coordinates of the points in the kernel of the isogeny. It is not clear to us if there are other ways of computing $x$-coordinates of the points in any specific subgroup of size $\ell$.

%We should avoid leaking the number of points on those elliptic curves over $\F_p$ and $\F_q$ with endomorphism ring $\OOO$. Otherwise the adversary can pick a random $x$ as the $x$-coordinate of a random point on the curve, and run Lenstra's factoring algorithm to factorize $N$. 

\subsubsection{Hiding the class group invariants}\label{sec:attack:basis}
In the applications of TGII, it is reasonable to assume that the closure of the gcd-compositions of the published $j$-invariants covers all the $h(D)$ $j$-invariants. So inverting a group element can be done by solving the discrete-log problem over $\CL(D)$.
However, the class number $h(D)$ is polynomially smooth, so the discrete-log problem over $\CL(D)$ can be solved in polynomial time once $h(D)$ is given, and $h(D)$ can be recovered from $D$ or any basis of a relation lattice of $\CL(D)$. So we do need to hide the discriminant $D$, the class number $h(D)$, and any lattice $\Lattice$ defined above. In the full version, we describe the details of how to hide these class group invariants.

Let us remark that if self-composition of an encoding is feasible, then one can efficiently guess all the polynomially smooth factors of $h(D)$. However for our construction self-composition is infeasible, due to the hardness of the $(\ell, \ell^2)$-isogenous neighbor problem.  Nevertheless, one can still attack by first guessing $D$ or $h(D)$, which takes $\secp^{O(\log\secp)}$ time according to the current setting of parameter.

%In the full version, we explain that $D$ and $h(D)$ are unlikely to be revealed directly from the curves and the splitting primes of $D$. Furthermore, to prevent leaking any full-rank basis of any of the relation lattice, we explain a way of choosing the prime ideals in the relation sets, and recommend to sample the exponent vectors  from a basis-independent distribution \cite{DBLP:conf/stoc/GentryPV08}.



%Finally, let us remark that if we were able to choose a super-polynomially large square-free discriminant $D$ with a trapdoor $\tau_D$, so that solving discrete-log over $\CL(D)$ is hard if one is given only $D$, but feasible if one is given the trapdoor $\tau_D$, then we can construct a system with $D$ and $h(D)$ being public, which would avoid all the complications in hiding $D$ and $h(D)$. 




%If a \emph{short} full-rank basis of $\Lattice_\OOO$ can be recovered then even if $|D|$ is large the system can be broken since it can be directly used to solve the discrete-log problem and get a short representation of the desirable group element. 


==> sec_broadcast_Irrer_etal.tex <==

\section{Broadcast encryption}

A broadcast encryption scheme allows the encrypter to generate ciphertexts that are decryptable by a designated subset of all the receivers. A trivial solution for broadcast encryption to simply encrypt the message for multiple times under the every user's decryption key. A meaningful broadcast encryption scheme requires an efficiency advantage over the trivial solution from either the cost of encryption, the size of the public parameters, or the sizes of the users' decryption keys \cite{DBLP:conf/crypto/FiatN93}. 

We give a concrete instantiation of the broadcast encryption scheme of Irrer et al. \cite{ILOP04} which was designed under the ideal interface of GII. Our instantiation supports private-key encryption, allows any numbers of users to collude. The encryption overhead and the users' secret keys are independent of the total number of the users $n$, but the public parameter size is linear in $n$. This is not the most efficient scheme in theory -- there are schemes which achieve $\log(n)$ public parameter overhead assuming the security of multilinear maps \cite{DBLP:conf/crypto/BonehWZ14} or iO \cite{DBLP:journals/iacr/Zhandry14a}. We leave the challenge of achieving $\log(n)$ public parameter blowup from (T)GII to the readers.


\begin{figure}
\begin{center}
\begin{tabular}{lllllll}\hline
Construction  						& $|\text{param}|$ & $|\text{user key}|$  & $|\text{CT}|$          & based on    & PK & CR \\\hline
\cite{DBLP:conf/crypto/FiatN93}     & $O(t^2 n \log n )$  & $O(t \log^2 t \log n)$ & $O(t^2 \log^2 t \log n)$ & RSA assumption           & No  & $\leq t$ users \\
%\cite{boneh2003applications} 		& $O(1)$  		   & $O(1)$  		      & $O(1)$ 	               & Ideal mmaps & No & Yes \\
\cite{ILOP04} 						& $O(n)$           & $O(1)$               & $O(1)$                 & Ideal GII   & No & Arbitrary \\
\cite{DBLP:conf/crypto/BonehGW05} I & $O(n)$           & $O(1)$               & $O(1)$                 & Bilinear maps & Yes & Arbitrary \\
\cite{DBLP:conf/crypto/BonehGW05} II& $O( \sqrt{n} )$  & $O(\sqrt{n})$        & $O(1)$                 & Bilinear maps & Yes & Arbitrary \\
\cite{DBLP:conf/crypto/BonehWZ14} 	& $O(\log n)$      & $O(\log n)$          & $O(\log n)$            & Mmaps 	& Yes & Arbitrary    \\
\cite{DBLP:journals/iacr/Zhandry14a}& $O(\log n)$      & $O(\log n)$          & $O(\log n)$            & iO 	& Yes & Arbitrary    \\
This work     						& $O(n)$           & $O(1)$               & $O(1)$                 & A concrete TGII & No  & Arbitrary  \\
\end{tabular}
\caption{A brief summary of the existing collusion resistant broadcast encryption schemes. $n$ represents the number of users; ``PK" stands for supporting public key encryption; ``CR" stands for being collusion resistant. All the parameters ignore the (possibly multiplicative) $\poly(\secp)$ factors. }
\end{center}
\end{figure}


\subsection{Definition}

A private-key broadcast encryption scheme consists of a tuple of efficient algorithms:
\begin{itemize}
\item $\Setup(1^\secp)$. The setup algorithm takes as input the security parameter $1^\secp$, generates the public parameters $\PP$, and the master secret key $\MSK$. 

\item $\Gen(\PP, \MSK, u)$. The user key generation algorithm includes the user ID $u$ in the list of users $\mathcal{U}$. It generates a secret key $\SK_u$ and possibly a public key $\PK_u$ for user $u$. $\PK_u$ is included in the public parameters.

\item $\Enc(\PP, \MSK, \Gamma, m)$. The encryption algorithm takes as input a polynomial size set $\Gamma \subseteq \mathcal{U}$ of recipients, produces (using $\PP, \MSK, \Gamma$) a key $K$ of a symmetric-key encryption scheme. Let $\CT_{K, m}$ be the encryption of the message $m$ under $K$. Outputs $\CT = (\Gamma, \CT_{K, m})$.

\item $\Dec(\PP, u, \SK_u, \CT)$. The decryption algorithm parses $\CT$ as $(\Gamma, \CT_{K, m})$, derives the symmetric-key $K$ from $\PP, \SK_u, \Gamma$, then uses $K$ to decrypt $\CT_{K, m}$.
\end{itemize}

The scheme is said to be correct if for all subsets of the users $\Gamma\subseteq\mathcal{U}$, for all messages $m$, a user $u$ from the set $\Gamma$ decrypts the correct message, i.e. $\Dec(\PP, u, \SK_u, \Gamma, \Enc(\PP, \MSK, \Gamma, m)) = m$. 

For security we consider the simplest form of the key-recovery attack, defined by the following game between an adversary and a challenger.
\begin{enumerate}
\item The challenger runs the setup algorithm to generate a master secret key $\MSK$ and the public parameters. Challenger then picks a set of users $\mathcal{U}$ and generates the public parameters and the users' decryption keys. The adversary is given $\mathcal{U}$ and the public parameters.
\item The adversary picks a subset $\Gamma \subseteq\mathcal{U}$ of receivers where it wants to attack. The challenger gives all users' keys $\SK_u$ for $u\notin\Gamma$.
\item The challenger runs the Encrypt algorithm to obtain $\Enc(\PP, \MSK, \Gamma, m)$. The adversary is given $\CT = (\Gamma, \CT_{K, m})$.
\item The adversary outputs a key $K'$ and wins the game if $K' = K$.
\end{enumerate}



\subsection{A private-key broadcast encryption scheme from TGII}

We first present the construction in the abstract syntax of a trapdoor group with infeasible inversion, then specify the detailed parameters in the instantiation using isogeny volcanoes.

\begin{construction}[Broadcast encryption under an abstract TGII]\label{cons:ideal}
Given a trapdoor group with infeasible inversion $\TGII$, a symmetric-key encryption scheme $\Sym$, construct a broadcast encryption scheme $\BE$ as follows.
\begin{itemize}
\item $\BE.\Setup(1^\secp)$. The setup algorithm takes as input the security parameter $1^\secp$, runs the TGII parameter generation algorithm to produce the public parameters $\TGII.\PP$ and the trapdoor $\tau$ of a group $\G = ( \circ, 1_\G )$. Then sample a random element $s\in\G$. 
The public parameter $\BE.\PP$ is set to be $\TGII.\PP$. 
The master secret key $\BE.\MSK$ includes $\tau$ and $s$.

\item $\BE.\Gen(\BE.\PP, \BE.\MSK, u)$: The user secret key generation algorithm parses $\tau, s$ from $\BE.\MSK$. It samples a random element $x\in\G$, computes $\enc(s \circ x)\la \TGII.\Trap\Sam(\TGII.\PP, \tau, s \circ x)$ as the user's public key $\PK_u$; computes $\enc( x)\la \TGII.\Trap\Sam(\TGII.\PP, \tau, x)$ and treat it as the user's secret key $\SK_u$.

\item $\BE.\Enc(\BE.\PP, \BE.\MSK, \Gamma)$: The encryption algorithm takes as input a polynomial size set $\Gamma \subseteq \mathcal{U}$ of recipients, computes the message encryption key $K$ as $K = \left( \prod_{i \in \Gamma} x_i \right)\circ s^{(|\Gamma|-1)} $. Compute $\Sym.\CT_{K, m}:= \Sym.\Enc(K, m)$. Outputs $\BE.\CT = (\Gamma, \Sym.\CT_{K, m})$.

\item $\BE.\Dec(\BE.\PP, u, \SK_u, \CT)$: The decryption algorithm extracts the set $\Gamma$ from $\BE.\CT$, takes the public keys $\PK_i$ for users $i\in\Gamma\setminus{u}$, the secret key $\SK_u$ for user $u$, computes $K' = \prod_{ i\in\Gamma\setminus{u} }(\PK_i)\circ \SK_u $, then decrypts $\Sym.\CT_{K, m}$ using $K'$.
\end{itemize}
\end{construction}

\paragraph{The instantiation from the concrete TGII and the choices of parameters.}
To instantiate the scheme based on the concrete TGII, the encryption algorithm use the canonical encoding of $K = \left( \prod_{i \in \Gamma} x_i \right)\circ s^{(|\Gamma|-1)} $ as the key for the symmetric encryption scheme. The decryption algorithm first computes the composable encoding of $K' = \prod_{ i\in\Gamma\setminus{u} }(\PK_i)\circ \SK_u $, then extract the canonical encoding of $K'$ as the symmetric decryption key (if the calculation is correct then $K' = K$).
As a more careful treatment, we can apply a randomness extractor on the $K$ so as to derive a key that is statistically close to the uniform distribution. 

As mentioned in the construction and the cryptanalysis sections (esp. Sections~\ref{sec:choices_param}~and~\ref{sec:attack_concrete_TGII}), we do not have a stateless universal solution for the distribution of the composable encodings. Here we provide the parameters for a broadcast encryption scheme where the master encryption algorithm is stateful. We give the details for the case where the group is $\CL(\OOO)_{\text{odd}}$ for a non-maximal order $\OOO$ (i.e. Choice~\ref{choice:II}). The case where the group is $\CL(\OOO)_{\text{odd}}$ for a maximal order $\OOO$ (Choice~\ref{choice:I}) follows analogously. 

\begin{itemize}
%\item Let $n$ be the expected total number of users. Update: we don't need to know $n$ ahead of time
\item Select $D_0<0$ of a large polynomial size (say $|D_0|\approx O(\secp^3)$) such that $h(D_0)$ is a prime. 
\item For the conductor $f$: choose a set $R$ of $2\log(\secp)$ primes such that for all $r\in R$, $\frac{r - \kron{D_0}{r} }{2}$ is a polynomially large prime of size $\approx O(\secp^3)$. Randomly pick $\log(\secp)$ numbers from $R$ and let them be $f_1, ..., f_{\log(\secp)}$. Set the conductor $f := \prod_{i\in [\log(\secp)]} f_i$. Let $\OOO$ be an order of discriminant $D = D_0\cdot f^2$ (choosing the factors of $f$ from a random subset of $R$ is mentioned as a safeguard in \S~\ref{sec:attack:basis}).

\item Let $m = O(\log(\secp))$. Pick a set of ideal classes $S = \set{ C_i = [(\ell_i, b_i, \cdot)] }_{i\in[m]}$ such that for all $i$, $[(\ell_i, b_i, \cdot)]$ generates $\CL(\OOO)_{\text{odd}}$, $5\leq \ell_i \leq \poly(\secp)$, and $\ell_i\notin R$.

\item To generate the master secret key, pick a random element $s\in\CL(\OOO)_{\text{odd}}$ using the class group invariants from the trapdoor (note that we do not need to compute any encodings of $s$).  

\item To generate each user $u$'s public key, choose a set of $m_u = O(\log^2(N))$ prime ideals $S_u = \set{ [( \ell_{u,i}, b_{u,i}, \cdot)] }_{i\in[m_u]}$ where the primes $\set{\ell_{u,i}}$ have never been used in the system. Then generates $\PK_u$ as a composable encoding of a random group element $x_u$ by running $\enc(x_u)\la\Random\Sam(\tau, S_u)$.

\iffalse
$x_u := \prod_i [(\ell_{u,i}, b_{u,i}, \cdot)]$. Let $\PK_u$ be the encoding of $x_u$ as 
\[ \PK_u = \enc(x_u) = (L; T_1, ..., T_{m_u} ) = ((\ell_{u,1}, ..., \ell_{u,m_u}), (j_{u, 1}), ..., (j_{u, m_u}) ), \]
where $j_{u, i}:= [(\ell_{u,i}, b_{u,i}, \cdot)] \cdot j_0 $. 
\fi

\item To generate each user $u$'s secret key, choose a set of $m'_u = O(\log^2(N))$ prime ideals $S'_u = \set{ [( \ell'_{u,i}, b'_{u,i}, \cdot)] }_{i\in[m'_u]}$ where the primes $\set{\ell'_{u,i}}$ have never been used in the system. Generates the composable encoding of a random group element $x'_u$: $\enc(x'_u)\la\Random\Sam(\tau, S'_u)$.

Next, solve the discrete-log problem of $s\circ x_u\circ (x'_u)^{-1}$ under the generation set $S$, obtain a short solution $\ary{e}_u\in\Z^m$ and derive from there the composable encoding of $s\circ x_u\circ (x'_u)^{-1}$. Then we obtain the secret key of user $u$ as a composable encoding of $s\circ x_u$: 
\[ \SK_u = \enc(s\circ x_u) = \comp(\PP, \enc(s\circ x_u\circ (x'_u)^{-1}), \enc(x'_u)).  \] 
\iffalse
\[ \SK_u = \enc(s\circ x_u) = 
((\ell_{1}, ..., \ell_{m}, \ell'_{u}), T_1, ...,  T_m, (j'_u) ), \]
where $j'_{u} = {x'_u}^{-1} \cdot j_0$; for $i\in[m]$, $T_{i} := ( j_{i,1}, ..., j_{i,e_{u,i} }  )$ where for $k\in[e_{u,i}]$, $j_{i}:= [(\ell_i, b_i, \cdot)]^k \cdot j_0$. 
\fi
\end{itemize}

Here all the public keys are encoded with relatively prime degrees. The encodings of secret keys do share common prime factors in their degrees, which does not create a problem for the decryption since the decryption algorithm only requires the composition of a secret key with many public keys (we can also encode the secret keys with relatively prime degrees).

In the encoding of user $u$'s secret key, we insert a random $x'_u$ with fresh prime ideal generators for two reasons. First it prevents trivially leaking an inverse of $\SK_u$. Note that solving discrete-log with the generation set $S$ could lead to negative entries in the exponent vector $\ary{e}\in\Z^m$. Without the fresh prime ideals in $\enc(x'_u)$, all the other generators in the encoding of $\SK_u$ are in the set $S$ shared with other users' secret keys, so the inverse might be trivially leaked in the other encodings of the secret keys. The prime ideals in $S'_u$ are only used once, which prevents trivially leaking any encoding of $(x'_u)^{-1}$.

The second reason is to prevent revealing any full-rank basis of a lattice $\Lattice'$ of dimension $m'$ such that $\Z^{m'}/\Lattice' \simeq \CL(\OOO)$ (i.e. to address the problem mentioned in Section~\ref{sec:attack:basis}). To wit, start from the following relation:
\[ \SK_{u_1}\circ \PK_{u_2}\circ ( \SK_{u_2}\circ \PK_{u_1} )^{-1} 
  = {x_1}\circ s \circ x_2 \circ ({x_2}\circ s \circ x_1)^{-1} = 1_{\CL(\OOO)}.  \]
This means if the users $u_1$ and $u_2$ collude, they can read off the exponents from the encodings of $\SK_{u_1}$, $\PK_{u_2}$, $\SK_{u_2}$ and $\PK_{u_1}$ to form a non-zero vector in the potential $\Lattice'$. Note that we are not computing a valid encoding of $( \SK_{u_2}\circ \PK_{u_1} )^{-1}$, which is supposed to be hard.

In general, let $n$ be the number of users in the system. We can obtain the vectors in some $\Lattice'$ from the exponents of the following relations:
\[  \SK_{u_1}\circ \PK_{u_i}\circ ( \SK_{u_i}\circ \PK_{u_1} )^{-1} 
  = {x_1}\circ s \circ x_i \circ ({x_i}\circ s \circ x_1)^{-1} , ~~\forall~ 2\leq i\leq n.\] 
It seems that all the non-trivial relations of $1_{\CL(\OOO)}$ can be obtained from the linear combinations of the $n-1$ vectors. So by enforcing distinct prime ideals in the encoding of each user's secret key, the dimension of the potential lattice $\Lattice'$ (i.e. the number of distinct prime degrees involved) is $(n-1)+ m + n \cdot O(\log(N))$, whereas the number of linearly independent zero relations is $n-1$. So it is not clear how to recover a full-rank basis of $\Lattice'$ from the encodings.

\begin{remark}
The CPA-style security definition in \cite{DBLP:conf/crypto/BonehGW05} requires that it is hard to distinguish a correct decryption key from a random key. Our scheme is also a candidate that satisfies the CPA definition when the decisional inversion problem is hard, which is plausible under the current setting of parameters.
\end{remark}

==> sec_missing_proofs.tex <==
\section{Proof of Theorem~\ref{thm:ratioD}}\label{sec:missingproof}

\begin{proof}[Proof of Theorem~\ref{thm:ratioD}]

We first give a lower bound on the number of ordinary elliptic curves over $\F_p$ whose endomorphism ring has discriminant $D$ such that $\kron{D}{\ell} = 1$. If for some pair of $(\ell, p)$ there are not enough elliptic curves over $\F_p$ with two horizontal $\ell$-isogenies then we count the elliptic curves with vertical $\ell$-isogenies.

We start with estimating the portion of $t\in [\ell]$ that satisfies $\kron{t^2 - 4p}{\ell} = 1$: 
\begin{equation}  
\Pr_{t\in[\ell]}\left[ \kron{t^2 - 4p}{\ell} = 1 \right] = 
\begin{cases}
	0 							& \ell = 2 \\
	\frac12-\frac{3}{2\ell}	& \ell > 2 \text{ and } \kron{4p}{\ell} = 1 \\
	\frac12- \frac{ 1}{2\ell}		& \ell > 2 \text{ and } \kron{4p}{\ell} = -1
\end{cases}
\end{equation} 
where the last two equations follows the identity\footnote{Derived from Theorem~19 in \url{http://www.imomath.com/index.php?options=328&lmm=0}.} $\sum_{t = 1}^{\ell} \kron{t^2 - 4p}{\ell} = -1$.
Hence for $\ell\geq 5$ or $\ell = 3$ and $\kron{4p}{3} = \kron{p}{3} = -1$, no less than $\frac12-\frac{ 3}{2\ell}$ of the $t\in[\ell]$ satisfy $\kron{t^2 - 4p}{\ell} = 1$. 

We now estimate the number of elliptic curves over $\F_p$ whose discriminant of the endomorphism ring $D$ satisfies $\kron{D}{\ell} = 1$. To do so we set $ r = \lfloor \sqrt{p} / \ell \rfloor $, and use Lemma~\ref{lemma:num_of_points_dist} by choosing the set $S$ as 
\[ S = \set{ s ~\bigg\vert \kron{(p+1-s)^2 - 4p}{\ell} = 1, s\in\set{ (p+1)-r\cdot\ell, ..., (p+1)+r\cdot\ell}\setminus\set{p+1}  }.  \]
Note that $\# S\geq r(\ell-3)$. 
Therefore, Lemma~\ref{lemma:num_of_points_dist}, there exists an effectively computable constant $c$ such that the number of isomorphism classes of elliptic curves over $\F_p$ with the number of points in the set $S$ is greater or equal to  
\begin{equation}\label{eqn:lenstra_bound}
 		 c\cdot (r(\ell-3)-2)\cdot \frac{\sqrt{p}}{\log p} 
	\geq c\cdot ((\frac{\sqrt{p}}{\ell}-1)(\ell-3)-2)\cdot \frac{\sqrt{p}}{\log p}
	> 	 c\cdot (\frac{\sqrt{p}}{2\ell} \cdot \frac{\ell}{3} - 2) \cdot \frac{\sqrt{p}}{\log p} 
	\geq c\cdot \frac{p}{ 18 \log p} . 
\end{equation}
Since the total number of elliptic curves over $\F_p$ is $p^2 - p$; the number of elliptic curves isomorphic to a given elliptic curve $E$ is $\frac{(p-1)}{\# \Aut E}$ \cite[(1.4)]{lenstra1987factoring}. 
So for $\ell\geq 5$ or $\ell = 3$ and $\kron{4p}{3} = -1$, the ratio of elliptic curves over $\F_p$ with discriminant $D$ such that $\kron{D}{\ell} = 1$ is $\Omega(\frac{1}{\log p})$.

To finish the treatment of the case, where $\ell\geq 5$, or $\ell = 3$ and $\kron{4p}{3} = \kron{p}{3} = -1$, we will show that among such curves the proportion of the $j$-invariants $j(E)$ on the crater of the volcano having one or two neighbors is $o(\frac{1}{\log p})$. Recall that we are in the case $\ell\nmid D$ and $\ell = \mathfrak{l}_1\mathfrak{l_2}$ in $\Q(\sqrt{D})$, and that the crater has size equals to the order of $\mathfrak{l}_1$ (which is the same as the order of $\mathfrak{l}_2$) in $\CL(\OOO)$. 

If the crater has $1$ or $2$ vertices, $\mathfrak{l}_1$ must have order dividing $2$ in $\CL(\OOO)$. If $\mathfrak{l}_1$ has order $1$ in $\CL(\OOO)$ then we have $x^2-Dy^2=\ell$ for some $x,y\in \Z$. Since $\ell$ is prime we necessarily have $y\neq0$. Moreover, since $6\ell<\sqrt{p}$ we have $-D<\sqrt{p}$ and therefore $4p -\sqrt{p}<t^2$. On the other hand, by the Hasse bound we have $t^2\leq 4p$, hence $4p-\sqrt{p}<t^2\leq4p$. Therefore, there are at most $O(p^{\frac14})$ $j$-invariants for which the the top of the volcano consists of a single vertex.  This handles the case of $\mathfrak{l}_1$ having order $1$.\\
The remaining case of $\mathfrak{l}_1$ having order $2$, on the other hand, cannot happen because of genus theory. More precisely, let $D_0$ be the discriminant of $\Q(\sqrt{D})$.  Since $\mathfrak{l}_1$ has order $2$ in $\CL(D)$ and $\mathfrak{l}_1\nmid D$ it has order $2$ in the class group $\CL(D_0)$ of $\Q(\sqrt{D})$. Now, recall that, by genus theory, the $2$-torsion in $\CL(D_0)$ is generated by primes dividing $D_0$. Therefore, if $\mathfrak{l}_1$ has order $2$, then $\mathfrak{l}_1\mid D_0$, which gives a contradiction.

Therefore, in the case of $\kron{D}{\ell}=1$ the probability that a random $j(E)\in \F_p$  having $\leq 2$ neighbors on the crater of the volcano is $O(p^{-\frac34})=o(\frac{1}{\log p})$, which finishes the treatment of the case $\ell\geq 5$ or $\ell = 3$ and $\kron{4p}{3} = \kron{p}{3} = -1$. 




For the remaining cases, where $\ell = 2$, or $\ell = 3$ and $\kron{p}{3} = 1$, we count the number of vertical isogenies. Following the formula for the depth of an isogeny volcano in Lemma~\ref{lemma:isograph}, for an elliptic curve $E(\F_p)$ of trace $t$ with $\ell^2\mid t^2 - 4p$, the curve lives on the part of the volcano of depth $\geq$ 1. In this case we only need to make sure that the curve does not live at the bottom of the volcano because otherwise it will necessarily have at least $\ell$-neighbors (if it is at the bottom it has only one neighbor). 

%When $\ell = 2$, if $t$ satisfies $4\mid t^2 - 4p$, then $4\mid (2t)^2 - 4p$. So every $t\in [ - \sqrt{q}, \sqrt{q}]\cap 2\Z$ corresponds to trace of an elliptic curve over $\F_p$ with at least two neighbors.

%When $\ell = 3$ and $\kron{p}{3} = 1$, if $t$ satisfies $9\mid t^2 - 4p$, then $9\mid (8t)^2 - 4p$. Once again, every $t\in [ - \sqrt{q}/4, \sqrt{q}/4]\cap \set{3\Z\pm 1}$ corresponds to the trace of an elliptic curve over $\F_p$ with at least two neighbors.

When $\ell = 2$, every $t=2t_1$ satisfies $4\mid t^2 - 4p$. So every $t\in [ - 2\sqrt{p}, 2\sqrt{p}]\cap 2\Z$ corresponds to trace of an elliptic curve over $\F_p$ with at least two neighbors.

When $\ell = 3$ and $\kron{p}{3} = 1$, Hensel's lemma implies that $\frac29$ of the $t\in [-2\sqrt{p},2\sqrt{p}]\cap\Z$  satisfy $t^2\equiv 4p \bmod 9$. These all correspond to traces of an elliptic curves over $\F_p$ with at least two neighbors.

Finally, in both cases using Lemma~\ref{lemma:num_of_points_dist} with a set $S$ that takes a constant fraction from $[ p+1-\sqrt{p}, p+1+\sqrt{p}]\cap\Z$, we see that the $O(\frac{1}{\log p})$ lower bound also applies for $\ell = 2$ or $\ell = 3$ and $\kron{p}{3} = 1$. 

\end{proof}

